Exploring the Role of Task Transferability in Large-Scale Multi-Task Learning

Recent work has found that multi-task training with a large number of diverse tasks can uniformly improve downstream performance on unseen target tasks. In contrast, literature on task transferability has established that the choice of intermediate tasks can heavily affect downstream task performance. In this work, we aim to disentangle the effect of scale and relatedness of tasks in multi-task representation learning. We find that, on average, increasing the scale of multi-task learning, in terms of the number of tasks, indeed results in better learned representations than smaller multi-task setups. However, if the target tasks are known ahead of time, then training on a smaller set of related tasks is competitive to the large-scale multi-task training at a reduced computational cost.

==> table.tex <==
	1
Single Task Model		2
Multihead Model 
Only SL		3
Multihead Model 
Only Glue		4
Multihead Model 
Only QA		5
Multihead Model 
SL + Glue		6
Multihead Model 
SL + QA		7
Multihead Model 
QA + Glue		8
Multihead Model 
QA + SL + Glue		9
Multihead Model NER
Dataset (train data size)	Avg	Std		Avg	Std		Avg	Std		Avg	Std		Avg	Std		Avg	Std		Avg	Std		Avg	Std		Avg	Std
WNUT 17 (3394)	63.239	0.332		63.124	0.651		43.461	1.857		60.623	1.857		59.729	1.253		64.261	0.797		57.56	3.622		64.359	0.577		65.248	0.68
Wikigold (1396)	80.409	1.437		83.449	0.166		72.174	8.055		78.173	1.044		81.403	0.511		83.114	0.571		76.023	1.214		81.635	0.991		80.343	0.625
NCBI Disease (5432)	86.849	0.463		87.069	0.558		85.412	0.596		86.456	0.866		87.037	0.433		87.458	0.328		86.642	0.703		87.378	0.733		86.801	0.432
MIT Movie EN (7996)	90.042	0.53		89.736	0.207		88.436	0.688		89.522	0.248		89.645	0.275		89.829	0.244		89.287	0.209		89.631	0.218		89.446	0.195
																										
BoolQ (9427)	73.804	1.158		70.761	0.726		78.313	0.488		77.14	0.712		78.457	0.503		76.427	0.814		80.147	0.271		79.515	0.517		71.184	0.563
CB (250)	86.333	4.201		82.121	5.179		87.161	1.079		68.93	10.657		84.336	4.201		85.003	3.925		80.638	10.67		89.565	2.165		67.853	16.113
COPA(400)	52.166	4.099		53.5	2.565		55.333	3.399		51.833	3.76		53.666	3.201		53.666	2.494		54.333	1.598		57.333	1.247		52.142	4.223
WiC(5428)	60.136	7.451		63.244	1.018		64.812	0.517		54.937	6.561		65.229	1.457		65.177	0.616		65.151	1.353		65.674	1.051		64.554	0.792
																										
Squad Adv (1424)	64.553	1.569		35.178	2.332		66.597	0.549		83.735	0.775		59.368	0.978		82.654	0.947		85.406	0.832		83.353	0.965		49.55	1.101
SubjQA (3276)	60.917	0.744		58.577	0.475		61.741	0.293		61.889	0.316		60.718	0.107		62.367	0.226		62.578	0.474		62.886	0.565		61.511	0.177
QED (7638)	37.779	5.495		36.544	1.169		51.604	1.345		74.643	0.445		46.533	1.217		77.196	0.51		73.91	1.42		76.312	0.824		34.161	0.308
Xquad - R	63.522	3.661		50.398	1.833		64.538	0.547		80.744	0.504		63.654	0.267		79.624	0.763		78.249	1.043		80.163	0.516		58.018	3.488
																										
Average of scores on unseen tasks	68.31242			64.47508			68.2985			72.38542			69.14792			75.56467			74.16033			76.48367			65.06758	
																										
Average of F1 scores on unseen SL tasks	80.13475			80.8445			72.37075			78.6935			79.4535			81.1655			77.378			80.75075			80.4595	
Average of scores on unseen Superglue tasks	68.10975			67.4065			71.40475			63.21			70.422			70.06825			70.06725			73.02175			63.93325	
Average of F1 scores on unseen QA tasks	56.69275			45.17425			61.12			75.25275			57.56825			75.46025			75.03575			75.6785			50.81	
																										
																										

